ParetoBandit: Budget-Paced Adaptive Routing for Non-Stationary LLM Serving

Multi-model LLM serving operates in a non-stationary, noisy environment: providers revise pricing, model quality can shift or regress without notice, and new models arrive regularly. More than a dozen recent methods have proposed learned routers to navigate the resulting quality--cost tradeoff across portfolios spanning a $\sim$530$\times$ cost range. Despite this activity, two gaps in the current solution space limit routing effectiveness under these conditions: no existing router enforces a dollar-denominated cost ceiling in closed loop over an open-ended request stream, and none provides principled online adaptation to post-deployment shifts in pricing or model quality. We present ParetoBandit, an open-source adaptive router built on cost-aware contextual bandits that addresses both gaps. Its core contributions are: (1) an online primal--dual budget pacer that enforces a per-request cost ceiling without a known horizon, and (2) geometric forgetting on sufficient statistics that gives the bandit bounded memory for tracking quality and cost shifts. A hot-swap model registry further supports runtime model changes with budget-controlled exploration. On 1,824 benchmark prompts with a three-model portfolio, the router maintains budget compliance within 0.4%, adapts to price and quality shifts with up to +0.071 quality lift, and integrates a cold-started model within $\sim$142 steps.

==> experiments/01_stationary_budget_pacing/table_budget_compliance.tex <==
\begin{table}[htbp]
\centering
\caption{Budget-paced routing results ($K{=}3$, 20~seeds).
  %
  \emph{\% Gemini Qual.}: mean reward as a percentage of
  Gemini-2.5-Pro's quality.
  \emph{Savings}: cost reduction relative to always calling
  Gemini-2.5-Pro.
  \emph{Util.}:\ mean realised cost / target $B$;
  bold values indicate binding targets
  (\bpUtilBindingLow--\bpUtilBindingHigh).
  $\lambda_{q50}$: median dual variable over the test phase.
  Fixed models are single-model baselines (no routing).
}
\label{tab:budget_compliance}
\small
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
\textbf{Budget}
  & \textbf{Reward}
  & \textbf{Cost}
  & \textbf{\% Gemini}
  & \textbf{Savings}
  & \textbf{Util.}
  & \textbf{$\lambda_{q50}$}
  \\
  &
  &
  & \textbf{Qual.}
  & \textbf{vs Gemini}
  &
  &
  \\
\midrule
\multicolumn{7}{@{}l}{\textit{Fixed single-model baselines}} \\[2pt]
Llama-3.1-8B & $0.793$ & $\$2.9\ensuremath{{\times}10^{-5}}$ & $85.1\%$ & $99.8\%$ & --- & ---  \\
Mistral-Large & $0.923$ & $\$5.3\ensuremath{{\times}10^{-4}}$ & $99.0\%$ & $96.5\%$ & --- & ---  \\
Gemini-2.5-Pro & $0.932$ & $\$1.5\ensuremath{{\times}10^{-2}}$ & $100.0\%$ & $0.0\%$ & --- & ---  \\
\\[-4pt]
\multicolumn{7}{@{}l}{\textit{BudgetPacer (adaptive)}} \\[2pt]
$B{=}\$2.9\ensuremath{{\times}10^{-5}}$ & $0.793\,[0.793,\,0.793]$ & $\$2.9\ensuremath{{\times}10^{-5}}$ & $85.1\%$ & $99.8\%$ & $\mathbf{0.98\times}$ & $2.86$  \\
$B{=}\$8.3\ensuremath{{\times}10^{-5}}$ & $0.813\,[0.812,\,0.814]$ & $\$8.3\ensuremath{{\times}10^{-5}}$ & $87.2\%$ & $99.5\%$ & $\mathbf{1.00\times}$ & $0.64$  \\
$B{=}\$2.3\ensuremath{{\times}10^{-4}}$ & $0.859\,[0.857,\,0.860]$ & $\$2.3\ensuremath{{\times}10^{-4}}$ & $92.1\%$ & $98.5\%$ & $\mathbf{1.00\times}$ & $0.46$  \\
$B{=}\$6.6\ensuremath{{\times}10^{-4}}$ & $0.898\,[0.894,\,0.901]$ & $\$6.5\ensuremath{{\times}10^{-4}}$ & $96.3\%$ & $95.7\%$ & $\mathbf{0.98\times}$ & $0.17$  \\
$B{=}\$1.9\ensuremath{{\times}10^{-3}}$ & $0.917\,[0.916,\,0.919]$ & $\$1.7\ensuremath{{\times}10^{-3}}$ & $98.4\%$ & $88.7\%$ & $0.91\times$ & $0.01$  \\
$B{=}\$5.3\ensuremath{{\times}10^{-3}}$ & $0.924\,[0.924,\,0.925]$ & $\$4.7\ensuremath{{\times}10^{-3}}$ & $99.2\%$ & $69.0\%$ & $0.89\times$ & $0.00$  \\
$B{=}\$1.5\ensuremath{{\times}10^{-2}}$ & $0.929\,[0.928,\,0.930]$ & $\$1.1\ensuremath{{\times}10^{-2}}$ & $99.7\%$ & $26.8\%$ & $0.74\times$ & $0.00$  \\
\bottomrule
\end{tabular}
\end{table}
